Metalic: Meta-Learning In-Context with Protein Language Models

Predicting the biophysical and functional properties of proteins is essential for in silico protein design. Machine learning has emerged as a promising technique for such prediction tasks. However, the relative scarcity of in vitro annotations means that these models often have little, or no, specific data on the desired fitness prediction task. As a result of limited data, protein language models (PLMs) are typically trained on general protein sequence modeling tasks, and then fine-tuned, or applied zero-shot, to protein fitness prediction. When no task data is available, the models make strong assumptions about the correlation between the protein sequence likelihood and fitness scores. In contrast, we propose meta-learning over a distribution of standard fitness prediction tasks, and demonstrate positive transfer to unseen fitness prediction tasks. Our method, called Metalic (Meta-Learning In-Context), uses in-context learning and fine-tuning, when data is available, to adapt to new tasks. Crucially, fine-tuning enables considerable generalization, even though it is not accounted for during meta-training. Our fine-tuned models achieve strong results with 18 times fewer parameters than state-of-the-art models. Moreover, our method sets a new state-of-the-art in low-data settings on ProteinGym, an established fitness-prediction benchmark. Due to data scarcity, we believe meta-learning will play a pivotal role in advancing protein engineering.

==> figs/barplot_template.tex <==
\usepackage{pgfplotstable}

% Helper macro to generate coordinates with error bars for each shot setting
\newcommand{\coordinateWithError}[3]{% #1=method, #2=mean, #3=stddev,
    (#1, #2) +- (#3, #3)
}

\newcommand{\spearmanBarPlot}[4]{ % #1, #2, #3 are data. #4 is boolean flag.

    % Combined bar plot for 0-shot, 16-shot, and 128-shot
    \begin{tikzpicture}
        \begin{axis}[
            ybar=0,
            symbolic x coords={PoET, \method, ESM1-v-650M, ESM2-8M, ProteinNPT},
            % xticklabels={\method, ESM1-v-650M, ESM2-8M, PoET, ProteinNPT}, % Apply \textit in xticklabels. When doing so, the order needs to be permuted this way to appear correctly and no idea why. Also, must set ProteinNPT data to NaN,NaN in Singles, but 0.0,NaN in multiples to show correctly.
            xtick=data,
            xticklabel style={rotate=45, anchor=east, xshift=4pt, yshift=-4pt}, % Rotate x labels
            ymin=0, 
            ymax={\ifnum#4=1 0.6 \else 1 \fi},
            bar width={\ifnum#4=1 0.8cm \else 0.265cm \fi}, % Conditionally adjust bar width
            % x= 1.1cm,
            % bar shift={\ifnum#4=1 .02cm \else 0cm \fi}, % Conditionally adjust x
            width=1.1\textwidth,
            height=6cm,
            % title={Spearman Correlation by Shot Setting},
            % title style={yshift=.1cm, font=\bfseries, color=black},
            % nodes near coords,
            % Move legend above the plot
            legend style={
                at={(0.51,.97)},
                anchor=north, % Place below the plot
                legend columns=-1, % Horizontal legend
                /tikz/every even column/.append style={column sep=0.5cm},
                % fill=gray!10,
                fill=none,
                draw=none,
            },
            every axis plot/.append style={draw=none},
            axis x line*=bottom, % Only show x-axis
            axis y line*=left,  % Show y-axis
            ymajorgrids=false, % Remove background grid
            % Background color
            % axis background/.style={
            %     fill=gray!10
            % },
            % Bar opacity
            every axis plot/.append style={fill opacity=0.8},
            % White grid lines
            grid=both,
            major grid style={line width=.5pt,draw=white},
            minor grid style={line width=.5pt,draw=white},
            xmajorgrids=false,
            xminorgrids=false,
            % Remove axis lines but keep ticks
            % axis line style={draw=none}, 
            % Major and minor tick lines style
            tick style={draw=white},
            % Manually format y-axis labels to remove leading zero
            yticklabel={
                \pgfmathparse{\tick < 1 && \tick > -1 ? \tick : int(\tick)}
                \ifdim\pgfmathresult pt=0pt
                    0
                \else
                    \ifdim\pgfmathresult pt<1pt
                        .\pgfmathparse{abs(\tick) * 10}%
                        \pgfmathprintnumber{\pgfmathresult}%
                    \else
                        \pgfmathprintnumber{\tick}%
                    \fi
                \fi
            },
            scaled y ticks=false,
        ]

        % Plot for 0-shot
        \addplot[
            ybar,
            % fill=blue!50,
            fill=blue!80!white,
            error bars/y dir=both, % Specify error bars in both directions
            error bars/y explicit, % Enable explicit error values
        ] coordinates {#1};
        \addlegendentry{0-Shot}

        % Plot for 16-shot
        \ifnum#4=0
        \addplot[
            ybar,
            % fill=orange!80,
            fill=orange!80!white,
            error bars/y dir=both, % Specify error bars in both directions
            error bars/y explicit, % Enable explicit error values
        ] coordinates {#2};
        \addlegendentry{16-Shot}
        \fi

        % Plot for 128-shot
        \ifnum#4=0
        \addplot[
            ybar,
            % fill=green!60,
            fill=green!65!gray,
            error bars/y dir=both, % Specify error bars in both directions
            error bars/y explicit, % Enable explicit error values
        ] coordinates {#3};
        \addlegendentry{128-Shot}
        \fi

        \end{axis}

    \end{tikzpicture}

% \end{figure}

}



==> figs/data_multiples.tex <==
% Define variables for each model and shot, in multiple mutants
\newcommand{\mMetalicZero}{.436}
\newcommand{\mMetalicZeroStd}{.011}
\newcommand{\mMetalicSixteen}{.484}
\newcommand{\mMetalicSixteenStd}{.001}
\newcommand{\mMetalicOneTwentyEight}{.670}
\newcommand{\mMetalicOneTwentyEightStd}{.003}
% Adjust Multi Data without Single Data
\newcommand{\mMetalicMultiTrainZero}{.376}
\newcommand{\mMetalicMultiTrainZeroStd}{.018}
\newcommand{\mMetalicMultiTrainHalfZero}{.307}
\newcommand{\mMetalicMultiTrainHalfZeroStd}{.022}
\newcommand{\mMetalicMultiTrainOneZero}{.047}
\newcommand{\mMetalicMultiTrainOneZeroStd}{.056}
% Adjust Multi Data with Single Data
\newcommand{\mMetalicMultiRestrictHalfZero}{.417}
\newcommand{\mMetalicMultiRestrictHalfZeroStd}{.021}
\newcommand{\mMetalicMultiRestrictOneZero}{.383}
\newcommand{\mMetalicMultiRestrictOneZeroStd}{.010}

% AuxIF
\newcommand{\mMetalicIFZero}{.480}
\newcommand{\mMetalicIFZeroStd}{.007}
\newcommand{\mMetalicIFSixteen}{.500}
\newcommand{\mMetalicIFSixteenStd}{.002}
\newcommand{\mMetalicIFOneTwentyEight}{.693}
\newcommand{\mMetalicIFOneTwentyEightStd}{.006}
% AuxIF Adjust Data
% 0-Shot
\newcommand{\mMetalicIFMultiTrainZero}{.533}
\newcommand{\mMetalicIFMultiTrainZeroStd}{.012}
\newcommand{\mMetalicIFMultiTrainHalfZero}{.517}
\newcommand{\mMetalicIFMultiTrainHalfZeroStd}{.021}
% The rest
\newcommand{\mMetalicIFMultiTrainSixteen}{.577}
\newcommand{\mMetalicIFMultiTrainSixteenStd}{.008}
\newcommand{\mMetalicIFMultiTrainOneTwentyEight}{.692}
\newcommand{\mMetalicIFMultiTrainOneTwentyEightStd}{.003}

\newcommand{\mESMvZero}{.426}
\newcommand{\mESMvZeroStd}{.000}
\newcommand{\mESMvSixteen}{.557}
\newcommand{\mESMvSixteenStd}{.000}
\newcommand{\mESMvOneTwentyEight}{.644}
\newcommand{\mESMvOneTwentyEightStd}{.000}

\newcommand{\mESMZero}{.368}
\newcommand{\mESMZeroStd}{.000}
\newcommand{\mESMSixteen}{.484}
\newcommand{\mESMSixteenStd}{.000}
\newcommand{\mESMOneTwentyEight}{.596}
\newcommand{\mESMOneTwentyEightStd}{.000}

\newcommand{\mPoETZero}{.588}
\newcommand{\mPoETZeroStd}{.014}
\newcommand{\mPoETSixteen}{.638}
\newcommand{\mPoETSixteenStd}{.001}
\newcommand{\mPoETOneTwentyEight}{.734}
\newcommand{\mPoETOneTwentyEightStd}{.006}

% \newcommand{\mProteinNPTZero}{N/A}
% \newcommand{\mProteinNPTZeroStd}{N/A}
% \newcommand{\mProteinNPTSixteen}{.382}
% \newcommand{\mProteinNPTSixteenStd}{.007}
% \newcommand{\mProteinNPTOneTwentyEight}{.621}
% \newcommand{\mProteinNPTOneTwentyEightStd}{.001}
% NPT with early stopping
\newcommand{\mProteinNPTSixteen}{.367}
\newcommand{\mProteinNPTSixteenStd}{.003}
\newcommand{\mProteinNPTOneTwentyEight}{.624}
\newcommand{\mProteinNPTOneTwentyEightStd}{.003}

==> figs/data_singles.tex <==
% Define variables for each model and shot, in single mutants
\newcommand{\sMetalicZero}{.482}
\newcommand{\sMetalicZeroStd}{.002}
\newcommand{\sMetalicSixteen}{.484}
\newcommand{\sMetalicSixteenStd}{.001}
\newcommand{\sMetalicOneTwentyEight}{.552}
\newcommand{\sMetalicOneTwentyEightStd}{.009}
% Ablations:
% zero-shot
\newcommand{\sMetalicNoICLZero}{.441}
\newcommand{\sMetalicNoICLZeroStd}{.002}
\newcommand{\sMetalicNoMetaZero}{-.046}
\newcommand{\sMetalicNoMetaZeroStd}{.018}
\newcommand{\sMetalicNoAugZero}{.464}
\newcommand{\sMetalicNoAugZeroStd}{.011}
\newcommand{\sMetalicNoPrefZero}{.465}
\newcommand{\sMetalicNoPrefZeroStd}{.011}
% 128-shot
\newcommand{\sMetalicNoFTOneTwentyEight}{.488}
\newcommand{\sMetalicNoFTOneTwentyEightStd}{.012}
\newcommand{\sMetalicNoICLOneTwentyEight}{.529}
\newcommand{\sMetalicNoICLOneTwentyEightStd}{.002}
\newcommand{\sMetalicNoMetaOneTwentyEight}{.346}
\newcommand{\sMetalicNoMetaOneTwentyEightStd}{.003}
\newcommand{\sMetalicNoAugOneTwentyEight}{.558}
\newcommand{\sMetalicNoAugOneTwentyEightStd}{.002}
\newcommand{\sMetalicNoPrefOneTwentyEight}{.520}
\newcommand{\sMetalicNoPrefOneTwentyEightStd}{.006}
% Additional Warmup exp:
\newcommand{\sMetalicWarmupOneTwentyEight}{.539}
\newcommand{\sMetalicWarmupOneTwentyEightStd}{.007}

\newcommand{\sMetalicIFZero}{.498}
\newcommand{\sMetalicIFZeroStd}{.008}
\newcommand{\sMetalicIFSixteen}{.500}
\newcommand{\sMetalicIFSixteenStd}{.002}
\newcommand{\sMetalicIFOneTwentyEight}{.556}
\newcommand{\sMetalicIFOneTwentyEightStd}{.005}

\newcommand{\sESMvZero}{.384}
\newcommand{\sESMvZeroStd}{.000}
\newcommand{\sESMvSixteen}{.452}
\newcommand{\sESMvSixteenStd}{.000}
\newcommand{\sESMvOneTwentyEight}{.553}
\newcommand{\sESMvOneTwentyEightStd}{.000}

\newcommand{\sESMZero}{.105}
\newcommand{\sESMZeroStd}{.000}
\newcommand{\sESMSixteen}{.226}
\newcommand{\sESMSixteenStd}{.000}
\newcommand{\sESMOneTwentyEight}{.406}
\newcommand{\sESMOneTwentyEightStd}{.000}

\newcommand{\sPoETZero}{.416}
\newcommand{\sPoETZeroStd}{.003}
\newcommand{\sPoETSixteen}{.475}
\newcommand{\sPoETSixteenStd}{.026}
\newcommand{\sPoETOneTwentyEight}{.588}
\newcommand{\sPoETOneTwentyEightStd}{.006}

\newcommand{\sProteinNPTZero}{N/A}
\newcommand{\sProteinNPTZeroStd}{N/A}
\newcommand{\sProteinNPTSixteen}{.192}
\newcommand{\sProteinNPTSixteenStd}{.003}
\newcommand{\sProteinNPTOneTwentyEight}{.443}
\newcommand{\sProteinNPTOneTwentyEightStd}{.003}
% Old (wthtout early stopping)
% \newcommand{\sProteinNPTSixteen}{.321}
% \newcommand{\sProteinNPTSixteenStd}{.009}
% \newcommand{\sProteinNPTOneTwentyEight}{.473}
% \newcommand{\sProteinNPTOneTwentyEightStd}{.002}
